Exploration of Helicon Plasmas for Wakefield Accelerators at the Madison AWAKE Prototype

Plasma wakefield accelerators have the potential to revolutionize particle physics by providing lepton collision energies orders of magnitude beyond current technology. Crucially, these accelerators require a high-density, highly homogeneous, scalable plasma source. The Madison AWAKE Prototype (MAP) is a new plasma development platform that has been built as part of CERN's beam-driven wakefield accelerator project AWAKE. MAP uses a dual helicon antenna setup with up to 20 kW of RF power to create plasmas in the low $10^{20}\,\mathrm{m^{-3}}$ range in a highly uniform magnetic field. The project is supported by a range of diagnostics that allow non-invasive measurements of plasma density, ion and neutral flows, and temperatures, and a 3D finite element model that can calculate helicon wavefield and power deposition patterns. In this paper, we present an in-depth overview of MAP's design and construction principles and main physics results. We show that the plasma discharge direction is set by the combination of antenna helicity and field direction and linked to the well-known preference for right-handed helicon modes. We find that the plasma density depends dramatically on the direction of plasma and neutral flow. A detailed measurement of the ionization source rate distribution reveals that most of the plasma is fueled radially by recycling at the wall, a finding with strong implications for optimizing plasma homogeneity. Lastly, we describe how helicon antennas can be engineered to optimize power coupling for a given target density. Together these findings pave the way toward the practical use of helicon plasmas in wakefield accelerators.

==> commandsV2.tex <==
\newcommand{\engU}[1]{[\mathrm{#1}]}
\newcommand{\U}[1]{\mathrm{\; #1}}
\newcommand{\E}[1]{\cdot 10^{#1}}
\newcommand{\Eb}[1]{10^{#1}}

\newcommand{\us}{$\U{\mu s}$}
\newcommand{\dens}{m^{-3}}

\newcommand{\ebd}[1]{\mathrm{10^{#1}\; m^{-3}}}
\newcommand{\ed}[1]{\mathrm{\cdot 10^{#1}\; m^{-3}}}

% === HIGHLIGHTING ===
% color highligted text
\newcommand{\hlcolor}[2]{\sethlcolor{#1}\hl{#2}}
\newcommand{\hg}[1]{\hlcolor{green}{#1}}
\newcommand{\hy}[1]{\hlcolor{yellow}{#1}}
\newcommand{\hb}[1]{\hlcolor{cyan}{#1}}
\newcommand{\ho}[1]{\hlcolor{red}{#1}}

%\renewcommand{\hlcolor}[2]{} % uncomment to disable all highlight commands
% \renewcommand{\hg}[1]{} % uncomment to disable \hg command
%\renewcommand{\hy}[1]{} % uncomment to disable \hy command
%\renewcommand{\hb}[1]{} % uncomment to disable \hb command
%\renewcommand{\ho}[1]{} % uncomment to disable \ho command

% color highligted picture boxes
\fboxrule=5pt
\newcommand{\cbox}[2]{\fcolorbox{#1}{white}{#2}}
\newcommand{\gbox}[1]{\cbox{green}{#1}}
\newcommand{\ybox}[1]{\cbox{yellow}{#1}}
\newcommand{\blbox}[1]{\cbox{cyan}{#1}}

\newcommand{\rf}{\hg{\textbf{[ref]}}}

\newcommand{\lifu}{$\U{\mu V s^{-1}}$}

% Insert picture
\newcommand{\pic}[4][1.0]{
\begin{figure}[htp]
	\begin{center}
		\includegraphics[width=#1\linewidth]{#2}
		\caption{#3}
		\label{#4}
	\end{center}	
\end{figure}}

% Insert picture with short hand description for list of figures
\newcommand{\lfpic}[5][1.0]{
\begin{figure}[htp]
	\begin{center}
		\includegraphics[width=#1\linewidth]{#2}
		\caption[#5]{#3}
		\label{#4}
	\end{center}	
\end{figure}}
